WavSpA: Wavelet Space Attention for Boosting Transformers' Long Sequence Learning Ability

Transformer and its variants are fundamental neural architectures in deep learning. Recent works show that learning attention in the Fourier space can improve the long sequence learning capability of Transformers. We argue that wavelet transform shall be a better choice because it captures both position and frequency information with linear time complexity. Therefore, in this paper, we systematically study the synergy between wavelet transform and Transformers. We propose Wavelet Space Attention (WavSpA) that facilitates attention learning in a learnable wavelet coefficient space which replaces the attention in Transformers by (1) applying forward wavelet transform to project the input sequences to multi-resolution bases, (2) conducting attention learning in the wavelet coefficient space, and (3) reconstructing the representation in input space via backward wavelet transform. Extensive experiments on the Long Range Arena demonstrate that learning attention in the wavelet space using either fixed or adaptive wavelets can consistently improve Transformer's performance and also significantly outperform learning in Fourier space. We further show our method can enhance Transformer's reasoning extrapolation capability over distance on the LEGO chain-of-reasoning task.

==> tex/method.tex <==
\section{\method}

As shown in Figure~\ref{fig:overview}(a), the only difference between a Transformer block and a \method block is the attention computation. 
In this section, we introduce the details that replace the attention computation in \method. 
The general flow of \paradigm is shown in Figure~\ref{fig:overview}(b), which constitutes the forward wavelet transform, the non-linearity in the middle, and the backward wavelet transform. 

We list our notations here --- we denote scalars as $x$, vectors as $\mathbf{x}$, matrices as $X$; we denote inner product between functions $f,g$ as $\langle f,g \rangle = \int f(t) g(t) \diff t$; we denote function $f$'s transformation in the coefficient space as $\hat{f}$. 

\paragraph{Background about Attention}
Let $X \in \mathbb{R}^{n\times d}$ denotes the input sequence of length $n$ and hidden dimension $d$. 
%A transformer block is a mapping from $\mathbb{R}^{n\times d}$ to $\mathbb{R}^{n\times d}$, constitutes an self-attention layer and an MLP layer as shown below:
A dense self-attention layer is shown below:
\begin{align}
    \mathrm{Attention}(X) &= \mathrm{Softmax}(\frac{Q K^\top}{\sqrt{d}}) V \label{eq:attn}
    %\mathrm{MLP}(X) &= \mathrm{ReLU}(X \cdot W_1 + b_1 ) \cdot W_2 + b_2 
\end{align}
%\zihan{there is another linear transformation between attention and MLP. Also not sure if you want to add the layernorms. I actually suggest to focus only on the self-attention part of the model and ignore the other parts.}
where $Q=X W_q$, $K=X W_k$, $V=X W_v$ with $W_q, W_k, W_v \in \mathbb{R}^{d \times m}$ stand for the query, key, and value, respectively.
The attention head size is denoted by $m$. 
The self-attention layer $\mathrm{Attention}(\cdot)$ computes a weighted average for each column of $V$ according to the dot-product similarity $QK^\top$ that is of $O(m n^2)$ number of operations.
% the root cause for the quadratic complexity in sequence length.


\subsection{Generalized Forward-Backward Paradigm}
We propose the generalized forward-backward paradigm to conduct learning in the coefficient space between forward and backward transformation. 
\paradigm is a special case of the generalized paradigm when the transformation is wavelet transform.
The forward transformation, also called analysis, decomposes the input sequence %\jingbo{what is ``the function''? is it better to say ``the input sequence''?} 
into coefficients of a set of orthogonal, complete functional basis.
We then conduct non-linear transformation in the coefficient space, which directly operates on the function. 
In the backward transformation, also called synthesis, we reconstruct the target representation in the original function space.

We require the forward-backward transformation pair to be invertible and exact, meaning that one can perfectly reconstruct the same input from the coefficients. 
Note that orthogonality is not necessary for this condition but a non-orthogonal basis cannot be transformed via simple inner product. 

The general framework is shown below. 
Without loss of generality, we limit ourselves to 1d functions. %for simplicity of our discussion.
Given input and output function $x(t), y(t) : \R \xrightarrow{} \R$ on time domain $t$, functional basis $g(\omega, t)$ on both time domain $t$ and frequency domain $\omega$, and non-linear transformation $F$. 
%\jingbo{may want to define what's $\omega$? the coefficient space variables/indices? can be frequency? also define $t$? the original input variables/indices? can be time?}
\begin{align}
    \mathrm{Forward\; Transform:} \quad \hat{x}(\omega) &= \int x(t) g^*(\omega, t)  \diff t = \sum_{i} x(t_i) g^*(\omega, t_i)\\
    \mathrm{Nonlinear\; Transform:}  \quad \hat{h}(\omega) &= F \circ \hat{x}(\omega)  \\
    \mathrm{Backward\; Transform:} \quad y(t) &= \int \hat{h}(\omega) g(\omega, t)  \diff \omega = \sum_j \hat{h}(\omega_j) g(\omega_j, t)
\end{align}
where $g^*(\omega, t)$ denotes the complex conjugate of $g$ in case $g$ has complex parts. 

As a concrete example, we use the Fourier transformation pair (formally defined in Appendix~\ref{sec:ft}) to illustrate this idea. 
Under Fourier transform, the functions are decomposed into sinusoidal waves, with $g(\omega, t)= e^{i 2\pi \omega t}$. 
The coefficients will represent the magnitude of the corresponding sinusoidal function. 
Hence, learning the mapping between any sequential function $x(t) \xrightarrow{} y(t)$ becomes learning a coefficient mapping between the transformed $\hat{x}(\omega) \xrightarrow{} \hat{y}(\omega)$ in a vector space. %, which can be effectively learned \jingbo{i'm not sure if ``can be effectively learned'' is neccessary or needs justification here. We can cite the vision transformer paper here?}. %by a simple multi-layer perceptron. 
%\yufan{We can get rid of the Fourier equations if needed} \jingbo{I think we should move the following two equations to Appendix. It should be something covered in textbook.}

In \paradigm, we utilize the more localized %\jingbo{do people usually say wavelet is more sophisticated? I feel it is easier to understand than Fourier...} \yufan{it's developed 100+ years later} 
wavelet transform as the forward-backward mechanism and in \method we use the random feature kernel as the non-linear transformation. 
However we want to highlight that numerous alternative candidates can fit in our generalized paradigm, we briefly list a few below.
For the forward-backward mechanism, any transformation based on orthogonal polynomials such as Chebyshev transform and Hartley transform will suit our purposes.
For the non-linear transformation, essentially any neural architecture with sufficiently strong learning power will be a valid candidate.

We will explain the inner workings of our \method's forward-backward transformation and the reason for choosing it in the next part.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{tex/img/ft_wt.pdf}
\vspace{-3mm}
\caption{We show a chirp signal from 1Hz to 4Hz on the left, its Fourier transform in the middle and its wavelet transform on the right. 
As you can see, from the Fourier transform graph one can only infer the existence of signal in the range of 1-4Hz without information on its happening time, while in the wavelet transform graph both time and frequency information are present and one can tell this is a chirp signal.}
\label{fig:FT_WT}
\vspace{-3mm}
\end{figure}

\subsection{Wavelet Transform}
Fourier transform decomposes the entire function into global sinusoidal waves. 
It tells people what \emph{frequencies} are there and in what \emph{magnitude}, but no information is given about \emph{when} that frequency started or ended. 
See Figure~\ref{fig:FT_WT} for an illustration on a chirp signal.
This limits the capability to understand the local structures of the input and to conduct learning on top of it, which is crucial to many machine learning tasks. 

%\jingbo{i think we want to mention Figure 2 in an earlier place like here.}

Wavelet transform is designed to solve this issue. 
It employs a function $\psi(x), x \in \R$, called mother wavelet, to generate a family of translated and dilated wavelets (see Figure~\ref{fig:overview}(b)): %\jingbo{refer to Figure 1(b) for visualizations. We can add i and j in the wavelet bases in Figure 1(b). Maybe just follow the same notation $\psi_{i,j}$ to each base?}
\begin{align}
    \psi_{i,j}(x) = 2^{\frac{i}{2}} \psi(2^i x - j),\quad i,j \in \mathbb{Z}
\end{align}
where scale $i$ controls the resolution %\jingbo{better say resolution? since we call it multi-resolution earlier?} 
of the wavelet and $j$ controls the position of the wavelet. 
With a larger $i$ the wavelet will be squeezed shorter in space, hence the normalization factor $2^{\frac{i}{2}}$ to ensure the same $L^2$ norm for all wavelets.
The wavelet family $\psi_{i,j}(x)$ is orthogonal on this dyadic grid.

To be a valid mother wavelet $\psi(x)$, the only requirement is admissibility:
\begin{align}
    \int_{\R} \psi(x) \diff x = 0
\end{align}
In other words, the sum of %\jingbo{is ``the sum of'' a more accurate description? } 
function value should be 0. 

Given any square integrable function $f \in \mathbb{L}^2(\R)$ (i.e., $\int |f(x)|^2 \diff x < \infty $) and wavelet functions $\psi_{i,j}$, the wavelet transform pair is defined as:
\begin{align}
    \mathrm{Forward\;Discrete\;Wavelet:} \quad &\hat{f}(i,j) = \int_{\R} f(x) \psi^*_{i,j}(x) \diff x = \sum_{t} f(x_t) \psi^*_{i,j}(x_t) \label{eq:dwtf}\\
    \mathrm{Backward\;Discrete\;Wavelet:} \quad &f(x) = \sum_{i=-\infty}^{+\infty} \sum_{j=-\infty}^{+\infty} \hat{f}(i,j) \psi_{i,j}(x)  \label{eq:dwtb}
\end{align}
where $\psi^*_{i,j}(x)$ denotes the complex conjugate of $\psi_{i,j}(x)$.

Intuitively, in wavelet transform, we are scanning $f(x)$ with a microscope that has two knobs. 
One knob is the location $j$, the other one is the frequency (i.e., $2^i$).
We will be able to oversee the local structure of the input and calibrate it accordingly with parameterized functions in \paradigm paradigm. See Figure~\ref{fig:FT_WT} for a direct comparison. 

To generalize beyond $\Lm^2(\R)$ and avoid using an infinite number of wavelets, we must introduce another function $\phi$, called scaling function with a similar admissibility and orthogonality constraint:
\begin{align}
    \int_{-\infty}^{+\infty} \phi(x) \diff x = 1,\quad \phi_{i,j}(x)= 2^{\frac{i}{2}} \phi(2^i x-j),\quad \textrm{s.t.} \langle \phi_{i,j}, \psi_{i',j'} \rangle = 0,\; i'>i,\;\forall j,j' 
\end{align}
$\phi_{i,j}$ is designed to cover the scale up to $i$, hence the orthogonality requirement. The decomposition of $f(x)$ therefore becomes:
\begin{align}
    f(x) = \sum_{j=-\infty}^{+\infty} \langle \phi_{0,j}, f \rangle \phi_{0,j}(x) + \sum_{i=0}^{+\infty}\sum_{j=-\infty}^{+\infty} \langle \psi_{i,j}, f \rangle \psi_{i,j}(x) \label{eq:mra}
\end{align}
Note that although $i$ still goes to $+\infty$ in (\ref{eq:mra}), $i$ usually has an upper limit in practice since it is impossible to work with infinite frequency. 
We also highlight that both the forward and backward discrete wavelet transform have an efficient $O(n)$ complexity algorithm~\citep{mallat1989theory}.

%\jingbo{do you mean $d$-dimensional space?}
In the $d$-dimensional case, we do not have a general orthogonal discrete $\R^d$ wavelet, unlike the continuous case. 
However, we can still perform discrete wavelet transform over each spatial dimension of the input, and we'd still be able to perfectly project and reconstruct the original function.

To summarize, wavelet transform enjoys $O(n)$ time complexity, an already desirable property compared to Fourier transform's $O(n\log n)$ complexity.
It further provides the capability to examine the local structures with different resolutions via altering the scale. %\jingbo{resolution?}. \yufan{common practice is to call this scale}
Learning carried out in this wavelet space will correspond to gathering and processing information from local to global level, in a coarse to fine-grained fashion. %similar to the design purpose of self-attention.

\subsection{Random Feature Kernel} \label{sec:random_feature_kernel}
We have explained the %\jingbo{not sure if we want to call it ``core''?} 
transformation mechanism for \paradigm. %\jingbo{I found that you like to use ``in the last part''. We probably can drop it or reduce its usage by assuming the readers will read the sections one by one.}
One question remains unanswered: which architecture should we choose to use as the parameterized non-linear transformation? 
For our purpose, the architecture should have linear complexity in sequence length; should be able to tackle sequential inputs effectively; should be as expressive as possible.
Among the ones that fit our criteria, we choose random feature kernel~\citep{rahimi2007randomkernel} due to its simplicity, efficiency, and theoretical benefits.

We have shown the self-attention in Equation~(\ref{eq:attn}). 
It can be rewritten using the softmax kernel (SM):
\begin{align}
    \mathrm{Softmax}(Q K^\top)_{i,j} = \frac{\mathrm{SM}(Q_i, K_j) }{\sum_{j=1}^{n} \mathrm{SM}(Q_i, K_j)}, \quad \mathrm{SM}(x, y) = \exp{(x^\top y)}
\end{align}
Random feature kernels aim to approximate $\mathrm{SM(\cdot, \cdot)}$ with randomized mapping $\nu: \R^d \xrightarrow{} \R^r_+$.
\begin{align}
    K(x,y) = \mathbb{E}[\nu(x)^\top \nu(y)]
\end{align}
We use FAVOR+ from Performer~\citep{performer} as the randomized mapping $\nu$:
\begin{align}
    \nu(x) = \frac{\exp{(-\frac{\|x\|^2}{2})}}{\sqrt{m}} (\exp{(w_1^\top x)}, \ldots, \exp{(w_m^\top x)}), \quad w_i \sim \mathcal{N}(0, \mathrm{I}_{d})\;\; \forall i \in \{1,\ldots,m\}
\end{align}
where $m$ denotes the number of random features. Similar to FAVOR+, we require $w_1,\ldots,w_m$ to be orthogonal to reduce the variance of estimation. However, we impose additional normalization on $x$ beforehand to further stabilize the estimation inspired by~\citet{random_feature_attention}. We note that this in-place normalization is important when bounding the MSE error of the random feature kernel, as shown in Appendix~\ref{sec:appendix_proof} Lemma~\ref{lemma:favor}.

%\jingbo{you may want to highlight that this normalization is also necessary as suggested by our later proof. I do have a question about the proof. Did Perform prove its universal approximating power? If so, how did they prove it without normalization?} \yufan{Peformer didn't talk about universal approximating power, they care about the case when $SM(x,y)$ is small, sinosoudal kernel will explode in this case but FAVOR+ won't}

%\begin{wrapfigure}{r}{0.5\textwidth}
%  \begin{center}
%  \includegraphics[keepaspectratio]{tex/img/pipeline.pdf}
%  \end{center}
%\caption{Pipeline Block}
%\label{fig:pipeline}
%\end{wrapfigure}

%\yufan{Explain the Complete Arch}

\subsection{Universal Approximation Power}
In this subsection, we show that \method has the same universal approximation power for seq-to-seq functions as Transformer.
The goal is to show that for any $f$ in $\mathcal{F}$, $\forall p \in [1, +\infty), \forall \epsilon >0$, we can find a $\bar{f}$ in the class of \method, such that:
%\jingbo{the norm notation seems wrong? you used a bracket on its right?}
\begin{align*}
    d_p(f, \bar{f}) = \left( \int_{\R^{n\times d}} \|f(\mathbf{X}) - \bar{f}(\mathbf{X})\|^p_p \diff \mathbf{X} \right)^{\frac{1}{p}} \leq \epsilon
\end{align*}

We define the \method class that has positional encoding, $h$ heads, head size $s$, hidden dimension $r$ as $\mathcal{W}^{h,s,r}$ with FAVOR+ kernel as described in Section~\ref{sec:random_feature_kernel}. 
\begin{theorem} \label{thm:main_theorem}
$\forall p \in [1, +\infty),\; \epsilon > 0$, and for any $f \in \mathcal{F}$, we can find a \method network $\mathsf{w} \in \mathcal{W}^{2,1,4}$, such that $d_p(f,\mathsf{w}) \leq \epsilon$. 
\end{theorem}
%\jingbo{$d_p$ not defined? p-norm distance?}

The sketch of the proof is simple: since we have required the transformation pair to be invertible and exact, so for any seq-to-seq function, we can universally approximate it in the wavelet space and it is equivalent to having universal approximation power in the original space.
The detailed proof of Theorem~\ref{thm:main_theorem} is shown in appendix~\ref{sec:appendix_proof}.


==> tex/method_backup.tex <==
\section{Waveformer}
In this section, we formalize our proposed \textit{\method}. 
We present that learning in wavelet coefficient space can be simple and efficient while enjoying universal approximating power for seq-to-seq functions.

We list our notations here: we denote scalars as $x$, vectors as $\mathbf{x}$, matrices as $X$; we denote inner product between functions $f,g$ as $\langle f,g \rangle = \int f(t) g(t) \diff t$; we denote function $f$'s transformation in the coefficient space as $\hat{f}$. 

\subsection{Dense Self-Attention}
Let $X \in \mathbb{R}^{n\times d}$ denotes the input sequence of $n$ tokens and $d$ hidden dimensions. 
%A transformer block is a mapping from $\mathbb{R}^{n\times d}$ to $\mathbb{R}^{n\times d}$, constitutes an self-attention layer and an MLP layer as shown below:
A self-attention layer is shown below:
\begin{align}
    \mathrm{Attention}(X) &= \mathrm{Softmax}(\frac{Q K^\top}{\sqrt{d}}) V \label{eq:attn}
    %\mathrm{MLP}(X) &= \mathrm{ReLU}(X \cdot W_1 + b_1 ) \cdot W_2 + b_2 
\end{align}
%\zihan{there is another linear transformation between attention and MLP. Also not sure if you want to add the layernorms. I actually suggest to focus only on the self-attention part of the model and ignore the other parts.}
where $Q=X W_q$, $K=X W_k$, $V=X W_v$ with $W_q, W_k, W_v \in \mathbb{R}^{d \times m}$ stands for the query, key and value. %, $W_1\in \mathbb{R}^{m\times r}$, $W_2 \in \mathbb{R}^{r\times d}$, $b_1 \in \mathbb{R}^r$, $b_2 \in \mathbb{R}^d$. 
The attention head size is denoted by $m$. %and the hidden layer size of the MLP is denoted by $r$. 
%We note that Transformers can have multiple attention heads, in that case, we will have separate set of parameters  $W_q^i, W_k^i, W_v^i,\; i\in \{1,\ldots,h\}$ for $h$ heads.

The self-attention layer $\mathrm{Attention}(\cdot)$ computes a weighted average for each column of $V$ according to the dot-product similarity $QK^\top$ that is of $O(m n^2)$ number of operations, the root cause for the quadratic complexity in sequence length.


\subsection{Generalized Forward-Backward Paradigm}
To tackle this problem, we propose the \textit{Generalized Forward-Backward Paradigm} to conduct learning in the coefficient space between forward and backward transformation. 
The forward transformation, also called analysis, decomposes the function into coefficients of an orthogonal complete functional basis.
We then conduct non-linear transformation in the coefficient space, which directly operates on the local and global parts of the function. 
In the backward transformation, also called synthesis, we reconstruct the target function in the original function space.

We require the forward and backward transformation pair to be exact, meaning that one can perfectly reconstruct the same input from the coefficients. Note that orthogonality is not necessary for this condition but non-orthogonal basis cannot be transformed via simple inner product. 

The general framework is shown as the following. 
Without loss of generality, we limit ourselves to 1d functions for simplicity of our discussion.
Given input and output function $x(t), y(t) : \R \xrightarrow{} \R$ , functional basis $g(\omega, t)$, and non-linear transformation $F$. 
\begin{align}
    \mathrm{Forward\; Transform:} \quad \hat{x}(\omega) &= \int x(t) g^*(\omega, t)  \diff t = \sum_{i} x(t_i) g^*(\omega, t_i)\\
    \mathrm{Nonlinear\; Transform:}  \quad \hat{h}(\omega) &= F \circ \hat{x}(\omega)  \\
    \mathrm{Backward\; Transform:} \quad y(t) &= \int \hat{h}(\omega) g(\omega, t)  \diff \omega = \sum_j \hat{h}(\omega_j) g(\omega_j, t)
\end{align}
where $g^*(\omega, t)$ denotes the complex conjugate of $g$ in case $g$ has any complex parts. 

As a concrete example, we use the Fourier transformation pair (shown in (\ref{eq:ff1}) and (\ref{eq:ff2})) to illustrate this idea. 
Under Fourier transform, the functions are decomposed into sinusoidal waves, with $g(\omega, t)= e^{i 2\pi \omega t}$. 
Therefore the coefficients will represent the magnitude of the corresponding sinusoidal function. 
Hence learning the mapping between any sequential function $x(t) \xrightarrow{} y(t)$ becomes learning a coefficient mapping between the transformed $\hat{x}(\omega) \xrightarrow{} \hat{y}(\omega)$ in a vector space, which can be effectively learned. %by a simple multi-layer perceptron. 
\yufan{We can get rid of the Fourier equations if needed}
\begin{align} 
    \mathrm{Forward\; Fourier:} \quad \hat{f}(\omega) &= \int_{-\infty}^{\infty} f(x) e^{-i 2\pi \omega x}  \diff x \label{eq:ff1} \\
    \mathrm{Backward\; Fourier:} \quad f(x) &= \int_{-\infty}^{\infty} \hat{f}(\omega) e^{i 2\pi \omega x}  \diff \omega \label{eq:ff2}
\end{align}
In \method, we utilize the more sophisticated wavelet transform as the forward-backward mechanism and the random feature kernel as the non-linear transformation. 
But we want to highlight that numerous other candidates will fit in our paradigm, we briefly list a few below.
For the forward-backward mechanism, any transformation based on orthogonal polynomials will suit our purposes such as Chebyshev transform and Hartley transform.
For the non-linear transformation, essentially any neural architecture with sufficiently strong learning power will work there.

We will explain the inner workings of our forward-backward transformation and the reason for choosing it in the next part.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{tex/img/ft_wt.pdf}
\vspace{-3mm}
\caption{We show a chirp signal from 1Hz to 4Hz on the left, its Fourier transform in the middle and its wavelet transform on the right. 
As you can see, from the Fourier transform graph one can only infer the existence of signal in the range of 1-4Hz without information on its happening time, while in the wavelet transform graph both time and frequency information are present and one can tell this is a chirp signal.}
\label{fig:FT_WT}
\vspace{-3mm}
\end{figure}

\subsection{Wavelet Transform}
As discussed in the last part, Fourier transform decomposes the entire function into global sinusoidal waves. 
It tells you what frequencies are there and in what magnitude but no information is given about when that frequency started or ended. %\yufan{Can add a graph here to show the difference}
This limits the ability to understand the local structures of the input and to conduct learning on top of it, which is crucial to many NLP tasks.

\textbf{Continuous Wavelet Transform}. \quad Wavelet transform is designed to solve this issue. 
It employs a function $\psi(\mathbf{x}), \mathbf{x} \in \R^n$, called mother wavelet, to generate a family of continuously translated and dilated wavelets:
\begin{align}
    \psi_{l,\mathbf{x}'}(\mathbf{x}) =  \frac{1}{l^{n/2}} \psi (\frac{\mathbf{x}-\mathbf{x}'}{l})
\end{align}
where $l\in \R^+$ denotes the scale of the wavelet and $\mathbf{x}' \in \R^n$ denotes the position of the wavelet. With a larger $l$ the wavelet will be stretched longer in space, hence the normalization factor $\frac{1}{l^{n/2}}$ to ensure the same $L^2$ norm for all wavelets.

To be a valid mother wavelet $\psi(\mathbf{x})$, the only requirement is admissibility:
\begin{align}
    \int_{\R^n} \psi(\mathbf{x}) \diff \mathbf{x} = 0
\end{align}
In other words, the average function value should be 0. 

Given any square integrable function $f \in \mathbb{L}^2(\R^n)$ (i.e., $\int |f(\mathbf{x})|^2 \diff \mathbf{x} < \infty $) and wavelet functions $\psi_{l,\mathbf{x}'}$, the wavelet transform pair is defined as:
\begin{align}
    \mathrm{Forward\;Wavelet:} \quad &\hat{f}(l,\mathbf{x}') = \int_{\mathbb{R}^n} f(\mathbf{x}) \psi^*_{l,\mathbf{x}'}(\mathbf{x}) \diff \mathbf{x} \label{eq:cwtf}\\
    \mathrm{Backward\;Wavelet:} \quad &f(\mathbf{x}) = C^{-1} \int_{\R^n} \int_{\R^+} \hat{f}(l,\mathbf{x}') \psi_{l,\mathbf{x}'}(\mathbf{x}) \frac{\diff l \diff \mathbf{x}'}{l^{n+1}} \label{eq:cwtb}
\end{align}
where $C=(2\pi)^n \int_{\R^n} |\hat{\psi}(\omega)|^2 \frac{\diff^n \omega}{|\omega|^n}$ indicates the normalizing factor, $\psi^*_{l,\mathbf{x}'}(\mathbf{x})$ denotes the complex conjugate of $\psi_{l,\mathbf{x}'}(\mathbf{x})$, and $\hat{\psi}(\omega)$ denotes the Fourier transform of $\psi(\mathbf{x})$.

Intuitively, in wavelet transform we are scanning $f(x)$ with a microscope that has two knobs. 
One knob is the location $x'$, the other one is the frequency (i.e., inverse of the scale $l$).
We will be able to oversee the local structure of the input and calibrate it accordingly with parameterized functions in the forward-backward paradigm. See Figure~\ref{fig:FT_WT} for a direct comparison. 

\textbf{Discrete Wavelet Transform}. \quad In continuous wavelet transform, the wavelets $\psi_{l,\mathbf{x}'}(\mathbf{x})$ constitutes a orthogonal complete set of $\Lm^2(\R^n)$, but we need to scan through all $l$ and $x'$. 
Is there a simpler way to only use a subset of $\psi_{l,\mathbf{x}'}(\mathbf{x})$ and retain orthogonality and completeness? 
The answer is yes if we limit ourselves in $\Lm^2(\R)$ and choose wavelet family $\psi_{i,j}(x)$ as below:
\begin{align}
    \psi_{i,j}(x) = 2^{\frac{i}{2}} \psi(2^i x - j),\quad i,j \in \mathbb{Z}
\end{align}
the wavelet family $\psi_{i,j}(x)$ is orthogonal on this dyadic grid. 
%We note that the discretized grid can be set in other ways with quasi-orthogonality
The forward and backward transform follow a similar structure as the continuous case:
\begin{align}
    \mathrm{Forward\;Discrete\;Wavelet:} \quad &\hat{f}(i,j) = \int_{\R} f(x) \psi^*_{i,j}(x) \diff x \label{eq:dwtf}\\
    \mathrm{Backward\;Discrete\;Wavelet:} \quad &f(x) = \sum_{i=-\infty}^{+\infty} \sum_{j=-\infty}^{+\infty} \hat{f}(i,j) \psi_{i,j}(x)  \label{eq:dwtb}
\end{align}
Note that the domain is limited to 1d square-integrable function space $\Lm^2(\R)$.

To generalize beyond $\Lm^2$ and avoid using infinite number of wavelets, we must introduce another function $\phi$, called scaling function with a similar admissibility constraint:
\begin{align}
    &\int_{-\infty}^{+\infty} \phi(x) \diff x = 1 \\
    &\phi_{i,j}(x)= 2^{\frac{i}{2}} \phi(2^i x-j),\quad \textrm{s.t.} \langle \phi_{i,j}, \psi_{i',j'} \rangle = 0,\; i'>i,\;\forall j,j' 
\end{align}
$\phi_{i,j}$ is designed to cover the scale up to $i$, hence the orthogonality requirement. The decomposition of $f(x)$ therefore becomes:
\begin{align}
    f(x) = \sum_{j=-\infty}^{+\infty} \langle \phi_{0,j}, f \rangle \phi_{0,j}(x) + \sum_{i=0}^{+\infty}\sum_{j=-\infty}^{+\infty} \langle \psi_{i,j}, f \rangle \psi_{i,j}(x) \label{eq:mra}
\end{align}
Note that although $i$ still goes to $+\infty$ in (\ref{eq:mra}), $i$ usually has an upper limit in practice since it is impossible to work with infinite frequency. 
We also highlight that both the forward and backward discrete wavelet transform have an efficient $O(n)$ complexity algorithm~\citep{mallat1989theory}.

In $n$-dimensional case, although we do not have a general orthogonal discrete $\R^n$ wavelet, unlike the continuous transform. 
We can still perform discrete wavelet transform over each spatial dimension of the input, and we'd still be able to perfectly project and reconstruct the original function.

To summarize, wavelet transform enjoys $O(n)$ time complexity, an already desirable property compared to Fourier transform's $O(n\log n)$ complexity.
It further provided the ability to examine the local structures with different resolutions via altering the scale. 
Learning carried out in this wavelet space will correspond to gathering and processing information from local to global level, in a coarse to fine-grained fashion, similar to the design purpose of self-attention.

\subsection{Random Feature Kernel}
We have explained the core transformation mechanism for \method in the last part. 
One question remains unanswered: which architecture should we choose to use as the parameterized non-linear transformation? 
For our purpose, the architecture should have linear complexity in sequence length; should be able to tackle sequential inputs effectively; should be as expressive as possible.
Among the ones that fit our criteria, we choose random feature kernel due to its simplicity, efficiency and theoretical benefits.

We have shown the self-attention in (\ref{eq:attn}), it can be rewrite using the softmax kernel (SM):
\begin{align}
    \mathrm{Softmax}(Q K^\top)_{i,j} = \frac{\mathrm{SM}(Q_i, K_j) }{\sum_{j=1}^{n} \mathrm{SM}(Q_i, K_j)}, \quad \mathrm{SM}(x, y) = \exp{(x^\top y)}
\end{align}
Kernel methods with random feature aim to approximate $\mathrm{SM(\cdot, \cdot)}$ with randomized mapping $\nu: \R^d \xrightarrow{} \R^r_+$ as shown below:
\begin{align}
    K(x,y) = \mathbb{E}[\nu(x)^\top \nu(y)]
\end{align}
We use FAVOR+~\citep{performer} as the backbone for randomized mapping $\nu$:
\begin{align}
    \nu(x) = \frac{\exp{(-\frac{\|x\|^2}{2})}}{\sqrt{m}} (\exp{(w_1^\top x)}, \ldots, \exp{(w_m^\top x)}), \quad w_i \sim \mathcal{N}(0, \mathrm{I}_{d})\;\; \forall i \in \{1,\ldots,m\}
\end{align}
where $m$ denotes the number of random features. Similar to FAVOR+, we require $w_1,\ldots,w_m$ to be exactly orthogonal to reduce the variance of estimation. However, we impose normalization on $x$ beforehand to further stabilize the estimation inspired by~\citet{random_feature_attention}.

\subsection{\method Block}

\jingbo{let's move this subsection to the beginning of this method section, serving as an overview. The reviewers should already have the general idea about the method after reading intro.}

After introducing the key forward-backward mechanism---wavelet transform, and the non-linear transformation---random feature kernel, we show the complete architecture in this subsection.

As shown in Figure~\ref{fig:pipeline}, one \method block constitutes the forward and backward wavelet transform, the normalization and the non-linearity in the middle. \yufan{TBD with more details}

%\begin{wrapfigure}{r}{0.5\textwidth}
%  \begin{center}
%  \includegraphics[keepaspectratio]{tex/img/pipeline.pdf}
%  \end{center}
%\caption{Pipeline Block}
%\label{fig:pipeline}
%\end{wrapfigure}

%\yufan{Explain the Complete Arch}

\subsection{Universal Approximation Power}
In this subsection, We show that \method has the same universal approximation power for seq-to-seq functions as Transformer.
The sketch of the proof is simple: since we have required the transformation pair to be exact, so for any seq-to-seq function, we can universally approximate it in the wavelet space and it is equivalent to having universal approximation power in the original space.
We define the function class $\mathcal{F}$ to be the set of all countinous functions that map a compact domain in $\R^{n\times d}$ to $\R^{n\times d}$. 
The end goal of the proof is to show that for any $f$ in $\mathcal{F}$, $\forall p \in [1, +\infty), \forall \epsilon >0$, we can find a $\bar{f}$ in the class of \method, such that:
\jingbo{the norm notation seems wrong? you used a bracket on its right?}
\begin{align*}
    d_p(f, \bar{f}) = \left( \int_{\R^{n\times d}} \|f(\mathbf{X} - \bar{f}(\mathbf{X}))^p_p \diff \mathbf{X} \right)^{\frac{1}{p}} \leq \epsilon
\end{align*}
We start from making the connection between random feature kernel and regular transformer block:
\begin{lemma} \label{lemma:favor}
(Asymptotic Result for FAVOR+ \jingbo{what's FAVOR+? if it refers to something in Performer, we may need some explanation and citation.}) The following is true for independent random $w_i$,
\begin{align*}
    & \mathrm{MSE}(\hat{\mathrm{SM}}(x ,y)) = \frac{1}{m} \exp{(\|x+y\|^2)} \mathrm{SM}^2(x,y) (1-\exp{(-\|x+y\|^2)}) \\
    \Rightarrow &\lim_{\mathrm{SM}(x,y)\xrightarrow{} 0} \mathrm{MSE}(\hat{\mathrm{SM}}(x ,y)) \xrightarrow{} 0
\end{align*}
where $\mathrm{SM}$ denotes the softmax kernel, $\hat{\mathrm{SM}}$ denotes the random feature kernel, and $\mathrm{MSE}$ stands for mean-squared error.
\end{lemma}
The proof of this lemma can be found at~\citet[Lemma 2]{performer}. 
It tells us the the MSE error is upper bounded to a constant since $x$, $y$ is normalized beforehand, and vanishes to 0 as the original softmax kernel value tends to 0 and the number of random features $m$ tends to $+\infty$. 

Next we use the main theorem of~\citet{yun2019transformers}. 
We denote the transformer network class that has positional encoding, $h$ heads, head size $s$, and hidden dimension $r$ as $\mathcal{T}^{h,s,r}$. 
\begin{lemma} \label{lemma:transformer}
$\forall p \in [1, +\infty),\; \epsilon > 0$, and for any $f \in \mathcal{F}$, we can find a Transformer network $g\in \mathcal{T}^{2,1,4}$, such that $d_p(f,g) \leq \epsilon$. 
\end{lemma}
The proof of Lemma~\ref{lemma:transformer} constitutes of several steps, of which the first step is to approximate any function $f \in \mathcal{F}$ as a piece-wise constant function $\Tilde{f}$.  
Since $f$ is continuous, the piece-wise constant approximation can be of arbitrary accuracy.
Next they find a modified transformer $\Tilde{g}$ with hardmax operator and a special class of activations. Finally they show that the transformer block $g$ is able to approximate $g$. The functional distance is then bounded by:
\begin{align*}
    d_p(f,g) \leq d_p(f,\Tilde{f}) + d_p(\Tilde{f}, \Tilde{g}) + d_p(\Tilde{g}, g) \leq \epsilon 
\end{align*}
We show that with slight modification, the proof will work for \method, and can be generalized to the Forward-Backward paradigm under certain constraints.

We define the \method class that has positional encoding, $h$ heads, head size $s$, hidden dimension $r$ as $\mathcal{W}^{h,s,r}$ with FAVOR+ kernel. 
\begin{theorem} \label{thm:main_theorem}
$\forall p \in [1, +\infty),\; \epsilon > 0$, and for any $f \in \mathcal{F}$, we can find a \method network $\mathsf{w} \in \mathcal{W}^{2,1,4}$, such that $d_p(f,\mathsf{w}) \leq \epsilon$. 
\end{theorem}
The proof is outlined below: 
For $\forall f \in \mathcal{F}$, its wavelet transform $\hat{f}$ (we will also use $f_w$ to denote this, see (\ref{eq:cwtf}) for details) is still continuous. 
Hence, the discretization claim remains valid. 
We can then effectively approximate the self-attention transformer block with the FAVOR+ block up to $\frac{\epsilon}{4}$ difference by controlling the number of random features $m$. In the end, the backward reconstruction is exact, the distance bound becomes when we control the other three terms to be less than $\frac{1}{4}\epsilon$ as well:
\begin{align*}
    d_p(f,\mathsf{w}) \leq d_p(f_w,\Tilde{f}_w) + d_p(\Tilde{f}_w, \Tilde{g}) + d_p(\Tilde{g}, g) + d_p(g, \mathsf{w}) \leq \epsilon \qed
\end{align*}


==> tex/motivation_old.tex <==
\section{Structured Associative Relationships and Attention Learning}
%\yufan{Motivation for Learning in transformed sequence space}
Attention was initially designed to learn associative relationships in human text~\cite{bahdanau2014neural}. Given ``\emph{how are \_\_}'', it learns to fill out ``\emph{you}''; given a piece of the news article, it learns to generate the summary of it. 
And naturally, such associative relationships can be multi-level since language is inherently complex and hierarchical. 
Textual information often consists of intertwined ideas and concepts organized at multi-level abstraction.

At a basic level, associative relationships can exist between individual words or phrases within a sentence. For example, consider the sentence: ``\emph{The cat chased the mouse.}'' 
Here, the words ``\emph{cat}'' and ``\emph{mouse}'' are associated with each other in terms of their roles in the action of chasing. 

The associative relationships can also extend beyond the sentence level. Natural texts are structured in paragraphs, sections, and documents where higher levels of association emerge. Within a paragraph, sentences can be associated with each other, playing different roles but conveying the same coherent idea. In a longer text, such as news articles or books, sections and chapters are arranged in a hierarchical manner, with associative relationships adhering them together under the same topic.

The multi-level nature of associative relationships in text reflects the complexity of human language and the way information is organized and conveyed. Moreover, this type of hierarchical structure exists in almost all kinds of sequential inputs. For example, source code has commands, functions, and classes, formulas have variables, operands, and theorems. Recognizing and understanding the multi-level hierarchy would give models the capacity to capture rich relationships present in the sequence, leading to more sophisticated sequential modeling capabilities.

%\jingbo{is it better to group the first few (above) paragraphs in this motivation part, and give it a small section name?} \yufan{I think so too}

To capture these multi-level associative relationships, we propose to learn attention in a transformed space, where the original sequence is decomposed into multiple levels such that the decomposition levels can encapsulate short-term or long-term relationships. We use wavelet transform as our transformation core, which has natural multi-level decomposition capabilities, and we dubbed the learning paradigm~\paradigm.






==> tex/table/code_glue.tex <==
\begin{wraptable}{R}{7cm}
  \begin{center}
    \label{tab:code_glue}
    \begin{tabular}{c|cc} 
      \toprule
      Model & Code-Defection & D2A-Function \\
      \midrule
      Code-BERT & 62.08  & 60.2 \\
      \midrule
      BERT-Medium & 59.69 & 59.73 \\
      \method & 61.38 & 62.58 \\
      \bottomrule 
    \end{tabular}
    
    \caption{Main results on Source Code Understanding Tasks.}
  \end{center}
\end{wraptable}




==> tex/table/code_glue_onetable.tex <==
\begin{figure}[t]
\begin{minipage}[c]{0.55\textwidth}
\centering
\small
\captionof{table}{Sequence length for each dataset's train split. The task of vulnerability detection requires reasoning over the entire piece of code snippet to deduct the label.}
\label{tab:code_glue_length}
\vspace{-3mm}
    \begin{tabular}{c|cc} 
      \toprule
      Dataset & CodeXGLUE & D2A-Func \\
      \midrule
      Average Length & 1277.49  & 1038.86\\
      \midrule
      Median Length & 561 & 717 \\
      \bottomrule 
    \end{tabular}
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}[c]{0.42\textwidth}
\centering
\small
\captionof{table}{Accuracy on vulnerability detection tasks. $\ssymbol{2}$ Evaluation on validation set. \label{tab:code_glue}}
\vspace{-1.8mm}
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc} 
      \toprule
      Model & CodeXGLUE & D2A-Func \\
      \midrule
      Code/C BERT & 62.08  & 60.2 \\
      \midrule
      BERT-medium & 59.69 & 59.73$\ssymbol{2}$ \\
      \method & 62.81 & 62.58$\ssymbol{2}$ \\
      \bottomrule 
    \end{tabular}
}
\end{minipage}
\vspace{-5mm}
\end{figure}


% \begin{wraptable}{r}{0.4\textwidth}
% \vspace{7mm}
% \small
% \parbox{\linewidth}{
% \caption{Sequence length for each dataset's train split. The task of vulnerability detection requires reasoning over the entire piece of code snippet to deduct the label.
% \label{tab:code_glue_length}}
%     \begin{tabular}{c|cc} 
%       \toprule
%       Dataset & CodeXGLUE & D2A-Func \\
%       \midrule
%       Average Length & 1277.49  & 1038.86\\
%       \midrule
%       Median Length & 561 & 717 \\
%       \bottomrule 
%     \end{tabular}

% }
% \vfill 
% \vspace{3mm}
% \parbox{\linewidth}{
% \caption{Accuracy on vulnerability detection tasks. $\ssymbol{2}$ Evaluation on validation set. \label{tab:code_glue}}
%     \begin{tabular}{c|cc} 
%       \toprule
%       Model & CodeXGLUE & D2A-Func \\
%       \midrule
%       Code/C BERT & 62.08  & 60.2 \\
%       \midrule
%       BERT-medium & 59.69 & 59.73$\ssymbol{2}$ \\
%       \method & 62.81 & 62.58$\ssymbol{2}$ \\
%       \bottomrule 
%     \end{tabular}
% }
% \vspace{-15mm}
% \end{wraptable}

==> tex/table/code_glue_stat.tex <==
\begin{wraptable}{R}{7cm}
  \begin{center}
    \label{tab:code_glue_length}
    \begin{tabular}{c|cc} 
      \toprule
      Dataset & Code-Defection & D2A-Function \\
      \midrule
      Average Length & 1277.49  & 1038.86\\
      \midrule
      Median Length & 561 & 717 \\
      \bottomrule 
    \end{tabular}
    
    \caption{Sequence length for each dataset's train split. The task of vulnerability detection requires reasoning over the entire piece of code snippet to deduct the label.}
  \end{center}
\end{wraptable}

==> tex/table/lego_table.tex <==
\begin{table}
  \begin{center}
    \caption{LEGO Table.}
    %\vspace{-3mm}
    \small
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccccc| cc} 
      \toprule
      Model &  15 & 16 & 17 & 18 & 19 & 20 & All & Test\\
      \midrule
      Transformer & 97.99 & 72.55 & 39.86 & 43.74 & 50.71 & 51.01  & 87.79 & 59.31 \\
      AdaWISE & 99.12 & 97.32 & 91.56 & 80.85 & 68.67 & 60.05 & 94.81 & 82.93 \\
      
      \bottomrule
    \end{tabular}
    %}
    
    \label{tab:lego_table}
  \end{center}
  %\vspace{-3mm}
\end{table}

==> tex/table/lego_table_oldformat.tex <==
\begin{table}
  \begin{center}
    \caption{LEGO Table.}
    %\vspace{-3mm}
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccccccccccccc|cccccc| cc} 
      \toprule
      Model &  1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & All & Test\\
      \midrule
      Transformer & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 99.99 & 99.96 & 97.99 & 72.55 & 39.86 & 43.74 & 50.71 & 51.01  & 87.79 & 59.31 \\
      AdaWISE & 100 & 100 & 100 & 100 & 100 & 99.89 & 99.95 & 99.92 & 99.89 & 99.89 & 99.88 & 99.83 & 99.74 & 99.64 & 99.12 & 97.32 & 91.56 & 80.85 & 68.67 & 60.05 & 94.81 & 82.93 \\
      
      \bottomrule
    \end{tabular}
    }
    
    \label{tab:lra_table}
  \end{center}
  %\vspace{-3mm}
\end{table}

==> tex/table/parameterization_table.tex <==
\begin{table}
  \begin{center}
    \caption{Evaluation results for the three adaptive parameterization schemes, we denote original space, direct/orthogonal parameterization, and wavelet lifting as N/A, Ada$\mathcal{W}$, Orth$\mathcal{W}$, and Lift$\mathcal{W}$.}
    %\vspace{-3mm}
    \small
    %\renewcommand\tabcolsep{3pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c | cccc | cccc | cccc | cccc | cccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{ListOps}} & \multicolumn{4}{c}{\textbf{Text}} & \multicolumn{4}{c}{\textbf{Retrieval}} & \multicolumn{4}{c}{\textbf{Image}} & \multicolumn{4}{c}{\textbf{Pathfinder}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
     & \textbf{N/A} & \textbf{Ada$\mathcal{W}$} & \textbf{Orth$\mathcal{W}$} & \textbf{Lift$\mathcal{W}$} & \textbf{N/A} & \textbf{Ada$\mathcal{W}$} & \textbf{Orth$\mathcal{W}$} & \textbf{Lift$\mathcal{W}$} & \textbf{N/A} & \textbf{Ada$\mathcal{W}$} & \textbf{Orth$\mathcal{W}$} & \textbf{Lift$\mathcal{W}$} & \textbf{N/A} & \textbf{Ada$\mathcal{W}$} & \textbf{Orth$\mathcal{W}$} & \textbf{Lift$\mathcal{W}$} & \textbf{N/A} & \textbf{Ada$\mathcal{W}$} & \textbf{Orth$\mathcal{W}$} & \textbf{Lift$\mathcal{W}$} \\
    \midrule
    \textbf{Trans.} & 36.37 & \textbf{\textcolor{ForestGreen}{55.40}} & \textcolor{ForestGreen}{45.95} & \textcolor{ForestGreen}{42.95} & 64.27 & \textcolor{ForestGreen}{81.60} & \textbf{\textcolor{ForestGreen}{81.63}} & \textcolor{ForestGreen}{75.63} & 57.46 & \textbf{\textcolor{ForestGreen}{79.27}} & \textcolor{ForestGreen}{71.52} & \textcolor{purple}{56.45} & 42.44 & \textbf{\textcolor{ForestGreen}{55.58}} & \textcolor{ForestGreen}{49.29} & \textcolor{ForestGreen}{42.48} & 71.40 & \textcolor{ForestGreen}{81.12} & \textcolor{ForestGreen}{81.13} & \textbf{\textcolor{ForestGreen}{81.73}} \\
    \textbf{Lin.} & 35.70 & \textcolor{ForestGreen}{37.15} & \textbf{\textcolor{ForestGreen}{38.05}} & \textcolor{ForestGreen}{37.30} & 53.94 & \textcolor{ForestGreen}{54.75} & \textbf{\textcolor{ForestGreen}{56.93}} & \textcolor{ForestGreen}{54.43} & 52.27 & \textcolor{ForestGreen}{61.09} & \textcolor{ForestGreen}{60.25} & \textbf{\textcolor{ForestGreen}{70.73}} & 38.47 & \textcolor{purple}{34.93} & \textbf{\textcolor{ForestGreen}{39.45}} & \textcolor{purple}{34.66} & 66.44 & \textcolor{purple}{65.66} & \textcolor{purple}{65.35} & \textcolor{purple}{63.49} \\
    \textbf{Linear.} & 16.13 & \textcolor{ForestGreen}{38.90} & \textbf{\textcolor{ForestGreen}{39.55}} & \textcolor{ForestGreen}{38.35} & 65.90 & \textcolor{ForestGreen}{76.82} & \textbf{\textcolor{ForestGreen}{79.45}} & \textcolor{ForestGreen}{73.39} & 53.09 & \textbf{\textcolor{ForestGreen}{71.38}} & \textcolor{ForestGreen}{69.65} & \textcolor{ForestGreen}{54.06} & 42.32 & \textbf{\textcolor{ForestGreen}{54.81}} & \textcolor{ForestGreen}{49.93} & \textcolor{ForestGreen}{44.39}  & 75.91 & \textbf{\textcolor{ForestGreen}{79.68}} & \textcolor{ForestGreen}{78.09} & \textcolor{purple}{74.46} \\
    \textbf{Long.} & 35.63 & \textbf{\textcolor{ForestGreen}{49.30}} & \textcolor{ForestGreen}{39.45} & \textcolor{ForestGreen}{39.40} & 62.85 & \textbf{\textcolor{ForestGreen}{79.73}} & \textcolor{ForestGreen}{78.41} & \textcolor{ForestGreen}{78.00} & 56.89 & \textcolor{ForestGreen}{58.57} & \textbf{\textcolor{ForestGreen}{79.93}} & \textcolor{purple}{53.27} & 42.22 & \textbf{\textcolor{ForestGreen}{50.84}} & \textcolor{ForestGreen}{49.93} & \textcolor{purple}{40.95} & 69.71 & \textbf{\textcolor{ForestGreen}{79.48}} & \textcolor{ForestGreen}{79.47} & \textcolor{ForestGreen}{75.80} \\
    \textbf{Per.} & 18.01 & \textbf{\textcolor{ForestGreen}{46.05}} & \textcolor{ForestGreen}{39.80} & \textcolor{ForestGreen}{39.85} & 65.40 & \textbf{\textcolor{ForestGreen}{80.93}} & \textcolor{ForestGreen}{79.10} & \textcolor{ForestGreen}{75.96} & 53.82 & \textbf{\textcolor{ForestGreen}{71.16}} & \textcolor{ForestGreen}{57.67} & \textcolor{purple}{52.75} & 42.77 & \textbf{\textcolor{ForestGreen}{52.06}} & \textcolor{ForestGreen}{48.78} & \textcolor{purple}{39.97} & 77.05 & \textcolor{ForestGreen}{77.17} & \textbf{\textcolor{ForestGreen}{78.09}} & \textcolor{purple}{76.20} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:adaptive_table}
  \end{center}
  \vspace{-6mm}
\end{table}

==> tex/table/parameterization_table_onepage.tex <==
\begin{table}
  \begin{center}
    \caption{Evaluation results for the three adaptive parameterization schemes, we denote direct/orthogonal parameterization, and wavelet lifting as Ada\paradigm, Ortho\paradigm, and Lift\paradigm.}
     %\jingbo{can we format this table to something similar to Table 1? Like every dataset has a few columns of results, N/A, Ada, Ortho, Lift? Resize the table a bit and it should save us some space too.}}
    \vspace{1mm}
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccccc|cc} 
      \toprule
      Models & ListOps & Text & Retrieval & Image & Pathfinder & Avg & Avg (w/r)\\
      \midrule
      \textbf{Transformer} & 36.37 & 64.27 & 57.46 & 42.44 & 71.40 & 54.39 & 53.62\\ 
      Ada\paradigm & \textbf{\textcolor{ForestGreen}{55.40}}	& \textcolor{ForestGreen}{81.60} & \textbf{\textcolor{ForestGreen}{79.27}} & \textbf{\textcolor{ForestGreen}{55.58}} &  \textcolor{ForestGreen}{81.12}  & \textbf{\textcolor{ForestGreen}{70.59}}	& \textbf{\textcolor{ForestGreen}{68.43}} \\
      Ortho\paradigm & \textcolor{ForestGreen}{45.95} & \textbf{\textcolor{ForestGreen}{81.63}} & \textcolor{ForestGreen}{71.52} & \textcolor{ForestGreen}{49.29} & \textcolor{ForestGreen}{81.13} & \textcolor{ForestGreen}{65.90} & \textcolor{ForestGreen}{64.50}\\
      Lift\paradigm & \textcolor{ForestGreen}{42.95} &	\textcolor{ForestGreen}{75.63} & \textcolor{purple}{56.45} & \textcolor{ForestGreen}{42.48} & \textbf{\textcolor{ForestGreen}{81.73}} & \textcolor{ForestGreen}{59.85}	& \textcolor{ForestGreen}{60.70} \\
      \midrule
      \textbf{Longformer} & 35.63 & 62.85 & 56.89 & 42.22 & 69.71 & 53.46 & 52.60 \\
      Ada\paradigm & \textbf{\textcolor{ForestGreen}{49.30}}	& \textbf{\textcolor{ForestGreen}{79.73}} & \textcolor{ForestGreen}{58.57} & \textbf{\textcolor{ForestGreen}{50.84}} &  \textbf{\textcolor{ForestGreen}{79.48}} & \textbf{\textcolor{ForestGreen}{63.66}} & \textbf{\textcolor{ForestGreen}{64.93}}\\
      Ortho\paradigm & \textcolor{ForestGreen}{39.45} & \textcolor{ForestGreen}{78.41} & \textbf{\textcolor{ForestGreen}{79.93}} & \textcolor{ForestGreen}{49.93} & \textcolor{ForestGreen}{79.47} & \textcolor{ForestGreen}{54.96} & \textcolor{ForestGreen}{54.96} \\
      Lift\paradigm & \textcolor{ForestGreen}{39.40} &	\textcolor{ForestGreen}{78.00} & \textcolor{purple}{53.27} & \textcolor{purple}{40.95} & \textcolor{ForestGreen}{75.80} & \textcolor{ForestGreen}{57.48} & \textcolor{ForestGreen}{58.54}\\
      \midrule
      \textbf{Performer} & 18.01 & 65.40 & 53.82 & 42.77 & 77.05 & 51.41 & 50.81 \\
      Ada\paradigm & \textbf{\textcolor{ForestGreen}{46.05}}	& \textbf{\textcolor{ForestGreen}{80.93}} & \textbf{\textcolor{ForestGreen}{71.16}} & \textbf{\textcolor{ForestGreen}{52.06}} &  \textcolor{ForestGreen}{77.17} & \textbf{\textcolor{ForestGreen}{65.47}} & \textbf{\textcolor{ForestGreen}{64.05}}\\
      Ortho\paradigm & \textcolor{ForestGreen}{39.80} & \textcolor{ForestGreen}{79.10} & \textcolor{ForestGreen}{57.67} & \textcolor{ForestGreen}{48.78} & \textbf{\textcolor{ForestGreen}{78.09}} & \textcolor{ForestGreen}{60.69}	& \textcolor{ForestGreen}{61.44} \\
      Lift\paradigm & \textcolor{ForestGreen}{39.85} & \textcolor{ForestGreen}{75.96} & \textcolor{purple}{52.75} & \textcolor{purple}{39.97} & \textcolor{purple}{76.20} & \textcolor{ForestGreen}{56.95} & \textcolor{ForestGreen}{58.00} \\
      \bottomrule
    \end{tabular}
    }
    
    \label{tab:adaptive_table}
  \end{center}
  \vspace{-6mm}
\end{table}

==> tex/table/time_table.tex <==
\begin{table}[ht]
  \begin{center}
    
    \label{tab:time_table}
    \begin{tabular}{c|cccc} 
      \toprule
      Model & 1000 & 2000 & 3000 & 4000 \\
      \midrule
      Transformer & 1 & 1 & 1 & 1 \\
      \midrule
      \method & 1.08x & 1.62x & 3.19x & 3.52x \\
      \bottomrule 
    \end{tabular}
    
    \caption{Main results on Long-Range Arena benchmark.}
  \end{center}
\end{table}
